Understanding the Impact of Adversarial Robustness on Accuracy Disparity

While it has long been empirically observed that adversarial robustness may be at odds with standard accuracy and may have further disparate impacts on different classes, it remains an open question to what extent such observations hold and how the class imbalance plays a role within. In this paper, we attempt to understand this question of accuracy disparity by taking a closer look at linear classifiers under a Gaussian mixture model. We decompose the impact of adversarial robustness into two parts: an inherent effect that will degrade the standard accuracy on all classes due to the robustness constraint, and the other caused by the class imbalance ratio, which will increase the accuracy disparity compared to standard training. Furthermore, we also show that such effects extend beyond the Gaussian mixture model, by generalizing our data model to the general family of stable distributions. More specifically, we demonstrate that while the constraint of adversarial robustness consistently degrades the standard accuracy in the balanced class setting, the class imbalance ratio plays a fundamentally different role in accuracy disparity compared to the Gaussian case, due to the heavy tail of the stable distribution. We additionally perform experiments on both synthetic and real-world datasets to corroborate our theoretical findings. Our empirical results also suggest that the implications may extend to nonlinear models over real-world datasets. Our code is publicly available on GitHub at https://github.com/Accuracy-Disparity/AT-on-AD.

==> broader_impact.tex <==
\section*{Broader Impact}
Trustworthy machine learning is a large ecosystem that contains multiple different yet closely-connected dimensions, including robustness, fairness, privacy, interpretability, etc. While each of these angles have been extensively studied in the literature, the interactions among them are less well-understood. 

In this work, we aim to rigorously characterize the interactions of adversarial robustness and fairness. Although we do not come up with any specific algorithm based on the theoretical findings, we do believe that a fundamental understanding will serve as a crucial ingredient in algorithmic advancement, and will eventually benefit the whole machine learning community by creating an integrated trustworthy framework --- which goes beyond targeting only one specific direction within.  

Finally, our work does not have direct
ethical or societal concerns due to its theoretical nature.


==> ridge.tex <==
\section{Accuracy Disparity in Ridge Regression}  \label{Section RR}
\han{Here when describing the setting, I changed the description that ``data consists of two classes'' to ``data come from two different groups'', mainly because that we are dealing with a regression problem and using the term class may confuse the readers in the sense that they may think the groundtruth label $y$ are binary.}
The connection between adversarial training and regularized linear regression pointed out in Section~\ref{subsection connection} motivates us to analyze accuracy disparity in regularized linear regression: while these two problems are not exactly equivalent due to the intercept term $b$ and the Gaussian assumption of data, it is still reasonable to expect a certain degree of similarity. Specifically, we raise the following hypothesis: 
\begin{align*}
    \textit{In linear regression, regularization will introduce accuracy disparity in presence of class imbalance. }
\end{align*}

We partially resolve the hypothesis with an affirmative answer in ridge regression.  It is worth emphasizing that the regularization term used in ridge is slightly different to the one in Eq. (\ref{Eq.optimization}) when $q=2$, mainly because we want to make the analysis trackable by considering a problem with closed-form solution.

The rest of this section is organized as follows:  we start by introducing the settings and notation, and formally state our goal. We proceed to show that no accuracy disparity exists in unregularized linear regression, and will present a key lemma that helps us characterize the population loss for different class. We will then move to ridge regression, and use a toy example to show why accuracy disparity arises in this context. Finally, we will present the general result, under which we will also discuss several implications and corollaries.  

\paragraph{Settings and Notation.} We consider the following regression problems:
\begin{align*}
   \bar{\beta} = \arg\min_\beta  \frac{1}{2N}\|Y-X\beta\|_2^2  \quad \text{and} \quad \hat{\beta} = \arg\min_\beta \frac{1}{2N}\|Y-X\beta\|_2^2 + \lambda \|\beta\|^2, 
\end{align*}
where the second one is exactly the ridge regression. Here $N$ is the number training instance, $X \in \mathbb{R}^{N \times d}$ is the design matrix, $Y \in \mathbb{R}^N$ is the label vector and $\beta \in \mathbb{R}^d $ is the estimator. 

Suppose the data come from two different groups: a majority group (Group $1$) and a minority class (Group $2$). We use $\nu_i$ to represent their corresponding data distributions, with mean $\mu_i$ and the same covariance matrix $\Sigma$. Within the design matrix, we assume there are $k_i$ instances coming from class $i$ ($i=1,2$), $k_1 + k_2 = N$, and $k_1/k_2 = K \gg 1$, i.e., $K$ represents the class imbalance ratio between these two groups. 

Finally, we assume the model is \textit{realizable}, i.e. there exists a $\beta^*$, such that 
\han{Actually, it has just come to my mind that the conclusion in this section holds under the following realizability assumption with the same $\beta^*$ being optimal simultaneously for both groups. However, one may argue that data from different groups may admit different optimal predictors, i.e., what if we still keep the realizability assumption but instead, assuming that for $X\sim G_1$, $y = \beta_1^{*\top}x$ whereas for $X\sim G_2$, $y = \beta_2^{*\top}X$? In this case, for our model, we can still solve for the same linear predictor $y\sim \beta^\top X$ since in most of the applications, the group identity of the data are protected and nonknown to the learner, so this justifies the choice of using the same $\beta$ for learning purpose. Will the high-level result in this section still hold in this more general setting?}
\begin{align*}
    y = \langle x, \beta^*  \rangle 
\end{align*}
gives the label of $x$ for all $x \in \text{class} \ 1 \cup \text{class}\  2$. Denote $n_i = \|\mu_i\|_2^2, m_i = \langle \mu_i, \beta^* \rangle$ ($i=1,2$).

\paragraph{Goal.} Our main interest lies in the following population loss for class $i$:
\begin{align} \label{Eq.loss}
    \ell_i(\beta) &= \mathbb{E}_{x\sim \nu_i} \frac{1}{2}\left(\langle x, \beta \rangle - \langle x, \beta^* \rangle\right)^2, \quad i=1,2.
\end{align}
\han{At this point, $\bar{\beta}$ and $\hat{\beta}$ have not been formally defined.}
We will analyze how accuracy disparity arises when we switch the measurement from $\bar{\beta}$ to $\hat{\beta}$ (i.e. the minimizers of ordinary linear regression and ridge regression), and how it relies on class imbalance which is reflected by $K$.

\subsection{Preparation work} \label{subsection RR_prep}
\han{The term ``unregularized linear regression'' is a bit non-standard, in the literature people use the term ``ordinary least square'' more often as it is known to most.}
We start with showing that unregularized linear regression treat both class equally in the low-dimensional regime, i.e. $d \le N$.
\han{This part is quite expected under the realizability assumption so I would change it from ``theorem'' to ``proposition'' so it does not diffuse readers' main focus.}
\begin{theorem}
Suppose $d \le N$ and $\nu_i$ ($i=1,2$) are continuous probability distribution, then $\bar{\beta} = \beta^*$ with probability one, which also implies
\begin{align*}
    \ell_1(\bar{\beta}) = \ell_2(\bar{\beta}) = 0.
\end{align*}
Therefore, there is no accuracy disparity. \han{I would imagine there is going to be an accuracy disparity under the more general setting that I mentioned above which then depends on the class imbalance factor $K$, even without explicit regularization in the OLS setting.}
\end{theorem}
\begin{proof}
Since $d \le N$ and $\nu_i$ ($i=1,2$) are continuous probability distribution, the design matrix $X$ has full column rank with probability one. This implies that the linear system $X\gamma = 0$ has unique solution. On the other hand, $\beta^*$ is obviously the optimal solution, so $\bar{\beta} = \beta^*$ with probability one. \han{Here the linear system should be the normal equation, not $X\gamma = 0$, right?}
\end{proof}
We then present a key lemma that characterizes the population loss for both classes, which helps simplify the analysis for ridge regression in the following subsections.

\begin{lemma} \label{Lemma tech}
Let $x=(x_i)$ be an $d \times 1$ random vector and let $A$ be an $d \times d$ symmetric matrix. If $\mathbb{E}[x]=\mu$ and  $\text{Var}[x]=\Sigma=(\sigma_{ij})$, then $\mathbb{E}[x^{\top}Ax]=\Tr(A\Sigma)+\mu^{\top}A\mu$.
\end{lemma}
The proof of Lemma \ref{Lemma tech} is deferred to Appendix \ref{Appendix RR_prep}. With this at hand, we can simplify the expression for $\ell_i(\beta)$ as follows:
\begin{align*}
    \ell_i(\beta) &= \mathbb{E}_{x\sim \nu_i} \frac{1}{2}\left(\langle x, \beta \rangle - \langle x, \beta^* \rangle\right)^2 \\
&= \frac{1}{2}\mathbb{E}_{x\sim \nu_i}x^{\top}(\beta-\beta^*)(\beta-\beta^*)^{\top}x \\
&=\frac{1}{2}\left(\Tr\left((\beta-\beta^*)(\beta-\beta^*)^{\top}\Sigma\right) + \mu_i^{\top}(\beta-\beta^*)(\beta-\beta^*)^{\top}\mu_i \right) \\
&=\frac{1}{2}\underbrace{(\beta-\beta^*)^{\top}\Sigma(\beta-\beta^*)}_{\text{Independent of } i} + \frac{1}{2}\underbrace{\mu_i^{\top}(\beta-\beta^*)(\beta-\beta^*)^{\top}\mu_i}_{\big|\langle \mu_i, \beta-\beta^*\rangle \big|^2}.
\end{align*}
Note the first term is independent of $i$, and the second term can be expressed as the square of $\big|\langle \mu_i, \hat{\beta}-\beta^*\rangle \big|$. Furthermore, the optimal solution for ridge regression~\cite{hastie2009elements} has the following form
\begin{align*}
    \hat{\beta} = (X^{\top}X + \lambda'I)^{-1}X^{\top}y = (X^{\top}X + \lambda'I)^{-1}X^{\top}X\beta^*,
\end{align*}
where $\lambda' = 2N\lambda$. Therefore, we will focus on studying the terms 
\begin{align*}
    \bigg|\big<\mu_i, \left((X^{\top}X + \lambda'I)^{-1}X^{\top}X - I\right)\beta^*\big>\bigg| \quad i= 1,2
\end{align*}
in the following analysis.

\subsection{Toy example} Here we will try to gain some intuitions on how accuracy disparity arises through the regularization term. To do so we will consider a toy example, in which the elements of the design matrix are directly sampled from the means $\mu_1$ and $\mu_2$, and we further assume $\langle \mu_1, \mu_2 \rangle =0$. 

Now 
\begin{align*}
    X^{\top}X = k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}
\end{align*}
is a rank-$2$ matrix, with non-zero eigenvalues being
\begin{align*}
    d_1^2 := \Tr(k_1\mu_1\mu_1^{\top}) = k_1n_1^2 \quad  \text{and} \quad d_2^2:=\Tr(k_2\mu_2\mu_2^{\top}) = k_2n_2^2
\end{align*}
since $\mu_1$ and $\mu_2$ are orthogonal. We use $X^{\top}X = VD^2V^{\top}$ to represent the singular value decomposition (SVD) of $X^{\top}X$, then 
\begin{align*}
    (X^{\top}X + \lambda'I)^{-1}X^{\top}X &= V(D^2+\lambda' I)^{-1}D^2V \\
&= \sum_{i=1}^2 v_iv_i^{\top}\frac{d_i^2}{d_i^2+\lambda'},
\end{align*}
where $v_i = \frac{\mu_i}{n_i}$ ($i=1,2$) are the normalized singular vectors. Therefore,
\begin{align*}
    \hat{\beta}- \beta^{*} = \left(\sum_{i=1}^2 \frac{k_i\mu_i\mu_i^{\top}}{k_in_i + \lambda'} - I\right)\beta^*,
\end{align*}
and
\begin{align*}
    \big|\langle \mu_i, \hat{\beta}-\beta^*\rangle \big| = \bigg|\frac{k_in_im_i}{k_in_i+\lambda'}-m_i\bigg| = \lambda'|m_i|\bigg|\frac{1}{k_in_i + \lambda'}\bigg|
\end{align*}
As a consequence, we have
\begin{align*}
    \big|\langle \mu_i, \hat{\beta}-\beta^*\rangle \big| = \Theta\left(\frac{1}{k_i}\right)
\end{align*}
if we treat all the rest parameters as constant.
So the observation here is that: \textbf{Ridge regression shrinks the principal components of $X$ according to their variance; the majority group corresponds to a direction with larger variance, so it will be shrunk less compared to the minority group --- which further results in a gap in accuracy.}

\subsection{General result} \label{subsection RR_general}
We will present the general result by gradually relaxing the constraints of the toy example in this subsection: we first consider the case where the means are not orthogonal, i.e., $n = \langle \mu_1, \mu_2 \rangle \neq 0$, but the data are still directly sampled from the means; then we further allow the data to come from a mixture of $\nu_i$.

We define the objectives of interest to be
\begin{align*}
    f_i(Z) := \mu_i^{\top}\left((Z^{\top}Z + \lambda'I)^{-1}Z^{\top}Z -I\right)\beta^*.
\end{align*}
Denote $S_Z = Z^{\top}Z$, we can further write $f_i(Z)$ as functions of the gram matrix $S_Z$
\begin{align*}
    g_i(S_Z) := f_i(Z) = \mu_i^{\top}\left((S_Z + \lambda'I)^{-1}S_Z -I\right)\beta^*.
\end{align*}
When the data are directly sampled from the means, the corresponding gram matrix for the design matrix $X$ is
\begin{align*}
    S := k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top};
\end{align*}
when the design matrix $Y$ (with each row being a data record $y_i^{\top}$) comes from a mixture of $\nu_i$, we assume w.l.o.g. that the first $k_1$ records come from class $1$ and the rest come from class $2$, and denote
\begin{align*}
    \epsilon_i := y_i - \mu_1, i \in [k_1]; \quad \delta_j := y_{k_1+j} - \mu_2, j \in [k_2].
\end{align*}
We write the gram matrix of $Y$ as $S' := Y^{\top}Y$.

\paragraph{Step 1: Relaxing the orthogonality constraint.} We will first consider a slightly relaxed scenario where the inner product $n$ is not zero. Following a similar approach as in the toy example, we will compute the SVD of the design matrix. The difference here is that we need to carefully bound the error term caused by the non-orthogonality. The main theorem is presented as follows, and we leave the details of proof to Appendix \ref{Appendix RR_general}.
\begin{theorem} \label{Theorem non-orthogonal}
Suppose $\lambda', n_1, n_2, m_1, m_2 = \Theta(1)$, $\mu_1$ and $\mu_2$ are not parallel, and $K \ge \frac{n_2}{n_1}\cdot s$ for some $s>1$. When the data are directly sampled from the means, we have
\begin{align*}
    g_1(S) \le O\left(\frac{1}{k_1}\right)+ O\left(\frac{k_2n^2+n}{k_1}\right),
\end{align*}
whereas
\begin{align*}
    g_2(S) \ge  \Omega\left(\frac{1}{k_2}\right) - O\left(\frac{k_2n^2}{k_1}\right) - O\left(\frac{n}{k_2}\right).
\end{align*}
\end{theorem}
As a consequence, we immediately have the following corollary.
\begin{corollary}
Suppose the conditions in Theorem \ref{Theorem non-orthogonal} hold, and we further assume the inner product satisfies 
\begin{align*}
   n \le O\left(\frac{1}{\sqrt{k_2}}\right), 
\end{align*}
then we have 
\begin{align*}
    g_1(S) \le O\left(\frac{1}{k_1}\right), \quad g_2(S) \ge  \Omega\left(\frac{1}{k_2}\right).
\end{align*}
\end{corollary}
\han{Add one sentence after this corollary to explicitly mention that ``in this case, the accuracy disparity is mainly due to the class imbalance, i.e., $O(1/k_1 - 1 / k_2)$''.}

\paragraph{Step 2: Relaxing the data constraint.}
Finally, we will relax the constraint of data by allowing them to come from a mixture of $\nu_i$. However, in this case it will be hard to directly characterize the objective functions $g_i(S')$, so we will instead analyze their surrogates: the \textit{first-order Taylor approximations} at $S$. Formally, define
\begin{align*}
    \widetilde{g_i}(S') := g_i(S) + \big< M_i, S'-S \big>,
\end{align*}
where 
\begin{align*}
    M_i := \left.\frac{\partial g_i(Z)}{\partial Z}\right|_{Z=S}.
\end{align*}
Our goal here is to build upon the results in Theorem \ref{Theorem non-orthogonal} and further estimate the first-order terms $\big< M_i, S'-S \big>$, which yield estimations for $\widetilde{g_i}(S')$ as in the following theorem.

\begin{theorem} \label{Theorem general_data}
Assume all the conditions in Theorem \ref{Theorem non-orthogonal} hold, and $\nu_i$ are sub-gaussian distributions with proxy-variance\footnote{This means that for all $v \in \mathbb{S}^{d-1}$ and random vector $X \sim \nu_i$, $v^{\top}X$ is a sub-gaussian random variable with parameter $\sigma^2$. As a special case, when $\nu_i$ follow the Gaussian distribution, $\sigma^2$ can be replaced by the operator norm of the covariance matrix, i.e. $\|\Sigma\|_2$. See~\cite{vershynin2018high} for more details.} $\sigma^2$. Then the first-order Taylor approximations of $g_i(S)$ at point $S$ satisfy
\begin{align*}
   |\tilde{g}_1(S')| \le O\left(\frac{1}{k_1}\right)+ O\left(\frac{k_2n^2+n}{k_1}\right) + O\left(\left(\sqrt{k_1d\sigma^2\log(1/\delta)} + (k_1+k_2)d\sigma^2\log(N/\delta)\right)\left(\frac{1}{k_1^2} + \frac{\sqrt{k_2}n}{k_1\lambda_2^{\frac{3}{2}}}\right)\right) 
\end{align*}
and
\begin{align*}
    |\tilde{g}_2(S')| \ge \Omega\left(\frac{1}{k_2}\right) - O\left(\frac{k_2n^2}{k_1}\right) - O\left(\frac{n}{k_2}\right) - O\left(\frac{{\sqrt{k_1d\sigma^2\log(1/\delta)} + (k_1+k_2)d\sigma^2\log(N/\delta)}}{\lambda_2^2}\right)
\end{align*}
with probability at least $1-O(\delta)$, where $\lambda_2$ is defined in Lemma \ref{Lemma eigen}.
\end{theorem}
With proper choices of $n$ and $\sigma^2$, we immediately obtain the following corollary.

\begin{corollary} \label{Corollary general}
Assume all the conditions in Theorem \ref{Theorem general_data} hold, and we further assume
\begin{align*}
    n \le \min\bigg\{O\left(\frac{1}{\sqrt{k_2}}\right), O\left(\frac{1}{K}\right)\bigg\}
\end{align*}
and
\begin{align*}
    \sigma^2 \le O\left(\frac{1}{dK\log N}\right),
\end{align*}
then with probability at least $1-O(\delta)$, 
\begin{align*}
    |\tilde{g}_1(S')| \le O\left(\frac{1}{k_1}\right) \quad \text{and} \quad |\tilde{g}_2(S')| \ge \Omega\left(\frac{1}{k_2}\right).
\end{align*}
\end{corollary}

\begin{proof}[Proof of Corollary \ref{Corollary general}]
It suffices to note that
\begin{align*}
    \sqrt{k_1d\sigma^2\log(1/\delta)} + (k_1+k_2)d\sigma^2\log(N/\delta) = O(k_2)
\end{align*}
when $\sigma^2 \le O\left(\frac{1}{dK\log N}\right)$, and 
\begin{align*}
    \lambda_2 \ge b-c = \Omega\left(k_2 - \sqrt{k_1k_2} n\right) = \Omega(k_2)
\end{align*}
when $n \le O\left(\frac{1}{K}\right)$.
\end{proof}

==> ridge_proof.tex <==
\section{Omitted Proof from Section \ref{Section RR}} \label{Appendix RR}
\subsection{Omitted Proof from Subsection \ref{subsection RR_prep}} \label{Appendix RR_prep}

\begin{proof}[Proof of Lemma \ref{Lemma tech}] We have
\begin{align*}
    \mathbb{E}[x^{\top}Ax] &= \sum_{i,j=1}^d a_{ij} \mathbb{E}[x_ix_j]\\
&=\sum_{i,j=1}^d a_{ij}(\sigma_{ij}+\mu_i\mu_j)\\
&=\sum_{i,j=1}^d a_{ij}\sigma_{ji} + \sum_{i,j=1}^da_{ij}\mu_i\mu_j\\
&=\Tr(A\Sigma) + \mu^{\top}A\mu.
\end{align*}

\end{proof}


\subsection{Omitted Proof from Subsection \ref{subsection RR_general}} \label{Appendix RR_general}
Our first step is to prove Theorem \ref{Theorem non-orthogonal}. To do this we need to introduce several technical lemmas.

\begin{lemma} \label{Lemma eigen}
Let $u, v \in \mathbb{R}^d$ satisfy $\langle u,v \rangle = c$ and $u \nparallel v$. Suppose $\|u\|_2^2 = a$ and $\|v\|_2^2 = b$. Then the non-zero eigenvalues for $A = uu^{\top} + vv^{\top}$ and their corresponding normalized eigenvectors are given by
\begin{align*}
    \lambda_1 = \frac{a+b +\sqrt{(a-b)^2 + 4c^2}}{2}, \quad \lambda_2 = \frac{a+b -\sqrt{(a-b)^2 + 4c^2}}{2}
\end{align*}
and
\begin{align*}
    v_1 = \frac{(\lambda_1-b)u+ cv}{\sqrt{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)}}, \quad v_2 = \frac{cu+(\lambda_2 - a)v}{\sqrt{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)}}.
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{Lemma eigen}]
Since $A$ is a rank-$2$ matrix, it has exactly two non-zero eigenvalues. Further, the eigenvectors of $A$ are the linear combinations of $u$ and $v$ and therefore has the form $pu+qv$. Comparing the coefficients of $u$ and $v$ in the following equation
\begin{align*}
    A(pu+qv) = \lambda(pu+qv)
\end{align*}
gives us
\begin{align*}
    \lambda^2 - (a+b)\lambda + (ab-c^2) = 0.
\end{align*}
Therefore, the non-zero eigenvalues of $A$ are given by
\begin{align*}
    \lambda_1 = \frac{a+b +\sqrt{(a-b)^2 + 4c^2}}{2}, \quad \lambda_2 = \frac{a+b -\sqrt{(a-b)^2 + 4c^2}}{2},
\end{align*}
and it is straightforward to compute their corresponding normalized eigenvector as
\begin{align*}
    v_1 = \frac{(\lambda_1-b)u+ cv}{\sqrt{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)}}, \quad v_2 = \frac{cu+(\lambda_2 - a)v}{\sqrt{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)}}.
\end{align*}
\end{proof}

\begin{lemma} \label{Lemma inequalities}
Following the notations in Lemma \ref{Lemma eigen}, we have the following inequalities: 
\begin{align*}
    \frac{\lambda_1}{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)} \le \frac{1}{(a-b)^2}, \quad \frac{\lambda_2}{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)} \le \frac{1}{(a-b)^2}.
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{Lemma inequalities}]
We have
\begin{align*}
   \frac{1}{(a^2-ab+2c^2) + \frac{(a-b)(c^2-ab)}{\lambda_1}} = \frac{1}{(a^2-ab+2c^2) - \frac{(a-b)(a+b-\sqrt{(a-b)^2+4c^2})}{2}} \le \frac{1}{(a-b)^2} 
\end{align*}
by setting $c^2 = 0$ in the last inequality. Similarly, 
\begin{align*}
   \frac{1}{(b^2-ab+2c^2) + \frac{(b-a)(c^2-ab)}{\lambda_2}} = \frac{1}{(b^2-ab+2c^2) + \frac{(a-b)(a+b+\sqrt{(a-b)^2+4c^2})}{2}} \le \frac{1}{(a-b)^2} 
\end{align*}
by setting $c^2=0$ in the last inequality. 
\end{proof}

\begin{lemma} \label{Lemma zero_one}
We have the following fact: for $0 \le x, y \le 1$,
\begin{align*}
    \max\{x,y\} \le 1 - (1-x)(1-y) \le x+y.
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{Lemma zero_one}]
We have
\begin{align*}
    1 - (1-x)(1-y) = x+y-xy \le x+y,
\end{align*}
and
\begin{align*}
    x+y-xy = x+(1-x)y \ge x, \quad x+y-xy = y+(1-y)x \ge y.
\end{align*}
\end{proof}

With this lemmas at hand, we are now ready to prove Theorem \ref{Theorem non-orthogonal}.

\begin{proof}[Proof of Theorem \ref{Theorem non-orthogonal}] We use the following notations:
\begin{align*}
    a := k_1n_1, b:=k_2n_2, c:=\sqrt{k_1k_2}n, u := \sqrt{k_1}\mu_1, v := \sqrt{k_2}\mu_2, I_1:=\langle u, \beta^* \rangle = \sqrt{k_1}m_1, I_2 := \langle v, \beta^* \rangle = \sqrt{k_2}m_2.
\end{align*}
The assumptions stated in the theorem directly implies that $a \ge bs$ for some $s > 1$, and that $c^2 < ab$.
Since the data are directly sampled from the means, we have
\begin{align*}
    X^{\top}X = u^{\top}u + v^{\top}v.
\end{align*}
Now we can apply SVD to $X^{\top}X$ using Lemma \ref{Lemma eigen}. Specifically, for the majority class we have
\begin{align*}
    \langle \mu_1, \hat{\beta}-\beta^*\rangle &= \bigg<\frac{u}{\sqrt{k_1}}, \left(\sum_{i=1}^2v_iv_i^{\top}\frac{\lambda_i}{\lambda_i + \lambda'} - I\right)\beta^*\bigg> \\
&= \frac{1}{\sqrt{k_1}}\left(\frac{\lambda_1}{\lambda_1+\lambda'}\cdot\frac{\left((\lambda_1-b)^2a + (\lambda_1-b)c^2\right)I_1 + \left((\lambda_1-b)ac + c^3\right)I_2}{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)}\right) \\
&  \ +\frac{1}{\sqrt{k_1}}\left(\frac{\lambda_2}{\lambda_2+\lambda'}\cdot\frac{c^2\lambda_2 I_1 + c\lambda_2(\lambda_2-a)I_2}{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)}\right) - \frac{1}{\sqrt{k_1}}I_1.
\end{align*}
The coefficient of $I_2$, which we denote as $C_2$, consists of two parts:
\begin{align*}
    \frac{(\lambda_1-b)ac + c^3}{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)}\cdot \frac{\lambda_1}{\lambda_1+\lambda'} \quad \text{and} \quad -\frac{c\lambda_2(a-\lambda_2)}{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)}\cdot \frac{\lambda_2}{\lambda_2+\lambda'}.
\end{align*}
Therefore,
\begin{align*}
    |C_2| &= \bigg|\left(\frac{c}{a-b}-\frac{2c^3\lambda_1}{(a-b)\left((a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)\right)}\right)\cdot\frac{\lambda_1}{\lambda_1+\lambda'} \\
   &\ - \left(\frac{c}{a-b}-\frac{2c^3\lambda_2}{(a-b)\left((b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)\right)}\right)\cdot\frac{\lambda_2}{\lambda_2+\lambda'}\bigg| \\
   &\le \frac{c}{a-b}\bigg|\frac{\lambda_1}{\lambda_1+\lambda'}-\frac{\lambda_2}{\lambda_2+\lambda'}\bigg| + \frac{2c^3}{(a-b)^3} \\
   &\le \frac{c\lambda'}{a-b}\frac{\sqrt{(a-b)^2+4c^2}}{ab-c^2} + \frac{2c^3}{(a-b)^3} \\
   &\le O\left(\frac{c\lambda'}{ab} + \frac{c^3}{(a-b)^3}\right),
\end{align*}
where we use Lemma \ref{Lemma inequalities} in the first inequality, the assumptions that $K \ge \frac{n_2}{n_1} \cdot s$ as well as $\mu_1$ and $\mu_2$ are not orthogonal in the last inequality. 

For the coefficient of $I_1$, which we denote as $C_1$, the dominated part can be estimated as
\begin{align*}
      1 - \frac{\lambda_1}{\lambda_1+\lambda'}\cdot\frac{(\lambda_1-b)^2a + (\lambda_1-b)c^2 }{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)} &= 1- \frac{\lambda_1}{\lambda_1+\lambda'}\cdot\frac{(a^2-ab+c^2)\lambda_1 + (a-b)(c^2-ab)}{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)} \\
   &\le \frac{\lambda'}{\lambda_1+\lambda'} + \frac{c^2\lambda_1}{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)} \\
   &\le \frac{\lambda'}{a+\lambda'} + \frac{c^2}{(a-b)^2}, 
\end{align*}
where we use Lemma \ref{Lemma zero_one} in the first inequality, Lemma \ref{Lemma inequalities} and the fact that $\lambda_1 \ge a$ in the last inequality. As for the secondary part, we can apply Lemma \ref{Lemma inequalities} again and bound it as
\begin{align*}
    \frac{\lambda_2}{\lambda_2+\lambda_2'}\cdot  \frac{c^2\lambda_2}{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)} \le \frac{c^2}{(a-b)^2}.
\end{align*}
Putting everything together and applying triangle inequality, we have
\begin{align*}
    \big|\langle \mu_1, \hat{\beta}-\beta^*\rangle \big| &\le O\left(\frac{\lambda'}{a+\lambda'} + \frac{c^2}{(a-b)^2}\right)\frac{|I_1|}{\sqrt{k_1}} + O\left(\frac{c\lambda'}{ab} + \frac{c^3}{(a-b)^3}\right)\frac{|I_2|}{\sqrt{k_1}} \\
   &= O\left(\frac{\lambda'}{k_1n_1+\lambda'} + \frac{k_1k_2n^2}{(k_1n_1-k_2n_2)^2}\right) + O\left(\frac{n\lambda'}{k_1n_1n_2} + \frac{k_1k_2^2n^3}{(k_1n_1-k_2n_2)^3}\right) \\
   &= O\left(\frac{1}{k_1}\right)+ O\left(\frac{k_2n^2+n}{k_1}\right).
\end{align*}
For the minority class, we have
\begin{align*}
    \langle \mu_2, \hat{\beta}-\beta^*\rangle &= \bigg<\frac{v}{\sqrt{k_2}}, \left(\sum_{i=1}^2v_iv_i^{\top}\frac{\lambda_i}{\lambda_i + \lambda'} - I\right)\beta^*\bigg> \\
   &= \frac{1}{\sqrt{k_2}}\left(\frac{\lambda_1}{\lambda_1+\lambda'}\cdot\frac{c\lambda_1(\lambda_1-b)I_1 + c^2\lambda_1I_2}{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)}\right) \\
   &  \ +\frac{1}{\sqrt{k_2}}\left(\frac{\lambda_2}{\lambda_2+\lambda'}\cdot\frac{\left(c^3+(\lambda_2-a)bc\right) I_1 + \left((\lambda_2-a)c^2+(\lambda_2-a)^2b\right)I_2}{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)}\right) - \frac{1}{\sqrt{k_2}}I_2.
\end{align*}
For the coefficient of $I_1$, which we denote as $C_1'$, we can do similarly as in the majority class and obtain the same estimation
\begin{align*}
    |C_1'| \le O\left(\frac{c\lambda'}{ab} + \frac{c^3}{(a-b)^3}\right).
\end{align*}
For the coefficient of $I_2$, which we denote as $C_2'$, the dominated part can be lower-bounded by 
\begin{align*}
    1-\frac{\lambda_2}{\lambda_2+\lambda'}\cdot\frac{\left((\lambda_2-a)c^2+(\lambda_2-a)^2b\right)I_2}{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)} \ge \frac{\lambda'}{\lambda_2+\lambda'} \ge \frac{\lambda'}{b+\lambda'}
\end{align*}
using Lemma \ref{Lemma zero_one}, whereas the secondary part can be upper-bounded by
\begin{align*}
    \frac{\lambda_1}{\lambda_1+\lambda'}\cdot\frac{c^2\lambda_1}{(a^2-ab+2c^2)\lambda_1 + (a-b)(c^2-ab)} \le \frac{c^2}{(a-b)^2}. 
\end{align*}
Putting everything together and applying triangle inequality, we have
\begin{align*}
    \big|\langle \mu_2, \hat{\beta}-\beta^*\rangle \big| &\ge \left(\frac{\lambda'}{b+\lambda'}-\frac{c^2}{(a-b)^2}\right)\frac{|I_2|}{\sqrt{k_2}} - O\left(\frac{c\lambda'}{ab} + \frac{c^3}{(a-b)^3}\right)\frac{|I_1|}{\sqrt{k_2}} \\
   &= \Omega\left(\frac{\lambda'}{k_2n_2+\lambda'}\right)-O\left(\frac{k_1k_2n^2}{(k_1n_1-k_2n_2)^2}\right) - O\left(\frac{n\lambda'}{k_2n_1n_2} + \frac{k_1^2k_2n^3}{(n_1k_1-n_2k_2)^3}\right) \\
   &= \Omega\left(\frac{1}{k_2}\right) - O\left(\frac{k_2n^2}{k_1}\right) - O\left(\frac{n}{k_2}\right).
\end{align*}
This finishes the proof of Theorem \ref{Theorem non-orthogonal} as desired.
\end{proof}

We will now proceed to prove two lemmas, which will serve as crucial ingredients in the proof of Theorem \ref{Theorem general_data}. 

\begin{lemma} \label{Lemma tech_data}
Following the same notations as in Theorem \ref{Theorem non-orthogonal}, we have
\begin{align*}
    \big\|\left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2}\mu_1\big\|_2 \le O\left(\frac{1}{k_1^2}\right) + O\left(\frac{\sqrt{k_2}n}{k_1\lambda_2^{\frac{3}{2}}}\right)
\end{align*}
and
\begin{align*}
    \big\|\left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2}\mu_2\big\|_2 \le O\left(\frac{1}{\lambda_2^2}\right).
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{Lemma tech_data}]
Using the SVD of the gram matrix, we have
\begin{align*}
    \left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2} = \frac{1}{(\lambda_1+\lambda')^2}v_1v_1^{\top} + \frac{1}{(\lambda_2+\lambda')^2}v_2v_2^{\top} + \sum_{k=3}^d\frac{1}{\lambda'^2}v_kv_k^{\top},
\end{align*}
where $v_k (3\le k \le d)$ correspond to the linearly independent normalized eigenvectors of the zero eigenvalue of $k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}$. Note
\begin{align*}
    v_1 \propto (\lambda_1-b)u+ cv, \quad v_2\propto  cu + (\lambda_2-a)v,
\end{align*}
and $v_i (i=1,2)$ are orthogonal to $v_k (3\le k \le d)$. Therefore, both $u$ and $v$ are orthogonal to $v_k (3\le k \le d)$. Now, 
\begin{align*}
    \left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2}\mu_1 = \frac{1}{\sqrt{k_1}}\left(\frac{1}{(\lambda_1+\lambda')^2}v_1v_1^{\top}u + \frac{1}{(\lambda_2+\lambda')^2}v_2v_2^{\top}u\right),
\end{align*}
so 
\begin{align*}
\big\|\left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2}\mu_1\big\|_2 &\le O\left(\frac{1}{\lambda_1^2}\right) + O\left(\frac{1}{\sqrt{k_1}(\lambda_2+\lambda')^2}\frac{c\lambda_2}{\sqrt{(b^2-ab+2c^2)\lambda_2 + (b-a)(c^2-ab)}}\right)\\
&\le O\left(\frac{1}{k_1^2}\right) + O\left(\frac{c}{\sqrt{k_1}\lambda_2^{\frac{3}{2}}(a-b)}\right) \\
&\le O\left(\frac{1}{k_1^2}\right) + O\left(\frac{c}{k_1^{\frac{3}{2}}\lambda_2^{\frac{3}{2}}}\right) \\
&= O\left(\frac{1}{k_1^2}\right) + O\left(\frac{\sqrt{k_2}n}{k_1\lambda_2^{\frac{3}{2}}}\right),
\end{align*}
where we use Lemma \ref{Lemma inequalities} in the second inequality. On the other hand,
\begin{align*}
\left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2}\mu_2 = \frac{1}{\sqrt{k_2}}\left(\frac{1}{(\lambda_1+\lambda')^2}v_1v_1^{\top}v + \frac{1}{(\lambda_2+\lambda')^2}v_2v_2^{\top}v\right),
\end{align*}
so
\begin{align*}
    \big\|\left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2}\mu_2\big\|_2 &\le O\left(\frac{1}{\lambda_1^2}\right) + O\left(\frac{1}{\lambda_2^2}\right) \\
    &\le O\left(\frac{1}{\lambda_2^2}\right).
\end{align*}

\end{proof}


\begin{lemma} \label{Lemma matrix}
Assume $P \in \mathbb{R}^{d \times d}$ is a positive semi-definite matrix and $B \in \mathbb{R}^{d \times d}$ be an arbitrary matrix, then
\begin{align*}
    \Tr(PB) \le \Tr(P)\|B\|_2.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{Lemma matrix}]
Denote $C = \|B\|_2 I - B$ and $D$ as the square root of $P$, i.e. $D^2 = P$. We then have
\begin{align*}
    \Tr(P)\|B\|_2 - \Tr(PB) = \Tr(PC) = \Tr(D^2C) = \Tr(D^{\top}CD) = \sum_{i=1}^d e_i^{\top}D^{\top}CDe_i.
\end{align*}
For arbitrary $x \in \mathbb{R}^d$, we have
\begin{align*}
    x^{\top}Cx = \|B\|_2\|x\|_2^2 - \|x^{\top}Bx\| \ge 0.
\end{align*}
Therefore,
\begin{align*}
    \Tr(P)\|B\|_2 - \Tr(PB) = \sum_{i=1}^d (De_i)^{\top}C(De_i) \ge 0.
\end{align*}
\end{proof}

We are now ready to prove Theorem \ref{Theorem general_data}.

\begin{proof}[Proof of Lemma \ref{Theorem general_data}]
Using Eq. (62) in~\cite{petersen2008matrix} and the chain rule, we have
\begin{align*}
    \frac{\partial g_i(Z)}{\partial Z} &= -(\lambda'I+Z)^{-1}\mu_i(\beta^*)^{\top}Z(\lambda'I+Z)^{-1} + (\lambda'I+Z)^{-1}\mu_i(\beta^*)^{\top}.
\end{align*}
Therefore,
\begin{align*}
    M_i &=\left[V(D^2+\lambda' I)^{-1}V^{\top}\right]\mu_i(\beta^*)^{\top}\left[V[I-D^2(D^2+\lambda' I)^{-1}]V^{\top}\right] \\
&= \lambda' \left[V(D^2+\lambda' I)^{-1}V^{\top}\right]\mu_i(\beta^*)^{\top}\left[V(D^2+\lambda' I)^{-1}V^{\top}\right],
\end{align*}
and
\begin{align*}
    \|M_i\|_2 &= \lambda'\bigg\|\left[V(D^2+\lambda' I)^{-1}V^{\top}\right]^2\mu_i(\beta^*)^{\top}\bigg\|_2 \\
&\lesssim \bigg\|\left[V(D^2+\lambda' I)^{-1}V^{\top}\right]^2\mu_i\bigg\|_2 \\
&= \big\|\left(k_1\mu_1\mu_1^{\top} + k_2\mu_2\mu_2^{\top}+\lambda'I\right)^{-2}\mu_i\big\|_2.
\end{align*}
On the other hand, denote 
\begin{align*}
     \epsilon:= \sum_{i\in[k_1]}\epsilon_i, \quad \delta :=\sum_{j\in[k_2]} \delta_j, \quad Q := \sum_{i\in[k_1]}\epsilon_i\epsilon_i^{\top} + \sum_{j\in[k_2]}\delta_j\delta_j^{\top},
\end{align*}
then 
\begin{align*}
    S' - S = {\epsilon\mu_1^{\top} + \mu_1\epsilon^{\top} + \delta\mu_2^{\top}+\mu_2\delta^{\top}+Q}.
\end{align*}
Therefore, by triangle inequality
\begin{align*}
    \big|\big< M_i, S'-S \big>\big| \le \big|\big< M_i, \epsilon\mu_1^{\top} \big>\big| + \big|\big< M_i, \mu_1\epsilon^{\top} \big>\big| + \big|\big< M_i, \delta\mu_2^{\top} \big>\big| + \big|\big< M_i, \mu_2\delta^{\top} \big>\big| 
+\big|\big< M_i, Q \big>\big|.
\end{align*}
For the first term on the right hand side, we have
\begin{align*}
    \big|\big< M_i, \epsilon\mu_1^{\top} \big>\big| = \big|\big<\epsilon, M_i\mu_1\big>\big| \le O\left(\|\epsilon\|_2\|M_i\|_2\right). 
\end{align*}
Note $\epsilon$ is the sum of $k_1$ i.i.d. sub-gaussian random vectors with proxy variance $\sigma^2$, so by the concentration of norm of sub-gaussian random vector~\cite{vershynin2018high}, we have
\begin{align*}
    \big|\big< M_i, \epsilon\mu_1^{\top} \big>\big| \le O\left(\sqrt{k_1d\sigma^2\log(1/\delta)}\|M_i\|_2\right)
\end{align*}
with probability at least $1-\delta$. Similarly, we have
\begin{align*}
    \big|\big< M_i, \mu_1\epsilon^{\top} \big>\big| \le O\left({\sqrt{k_1d\sigma^2\log(1/\delta)}}\|M_i\|_2\right), \quad \big|\big< M_i, \delta\mu_2^{\top} \big>\big|\le O\left({\sqrt{k_2d\sigma^2\log(1/\delta)}}\|M_i\|_2\right),
\end{align*}
and
\begin{align*}
    \big|\big< M_i, \mu_2\delta^{\top} \big>\big|\le O\left({\sqrt{k_2d\sigma^2\log(1/\delta)}}\|M_i\|_2\right).
\end{align*}
Finally, for the last term in the right hand side, we have
\begin{align*}
    \big|\big< M_i, Q \big>\big| = \Tr(QM_i) \le \Tr(Q)\|M_i\|_2, %
\end{align*}
where we apply Lemma \ref{Lemma matrix} in the inequality. Note
\begin{align*}
    \Tr(Q) = \sum_{i \in [k_1]}\|\epsilon_i\|_2^2 + \sum_{j\in [k_2]}\|\delta_j\|_2^2,
\end{align*}
so we can again apply the concentration of norm of sub-gaussian random vector, as well as a union bound to obtain
\begin{align*}
    \big|\big< M_i, Q \big>\big| \le (k_1+k_2)d\sigma^2\log(N/\delta)\|M_i\|_2.
\end{align*}
Finally, we can combine Theorem \ref{Theorem non-orthogonal} and Lemma \ref{Lemma tech_data} which gives us estimations of $\|M_i\|_2$, to obtain the desired results.
\end{proof}
